State Complexity of Permutation and Related Decision Problems on Alphabetical Pattern Constraints

We investigate the state complexity of the permutation operation, or the commutative closure, on Alphabetical Pattern Constraints (APC). This class corresponds to level $3/2$ of the Straubing-Th{\'e}rien Hierarchy and includes the finite, the piecewise-testable, or $\mathcal J$-trivial, and the $\mathcal R$-trivial and $\mathcal L$-trivial languages. We give a sharp state complexity bound expressed in terms of the longest strings in the unary projection languages of an associated finite language and which is already sharp for the subclass of finite languages. Additionally, for two subclasses, we give sharp bounds expressed in terms of the size of a recognizing input automaton and the size of the alphabet. Lastly, we investigate the inclusion and universality problem on APCs up to permutational equivalence, two problems known to be PSPACE-complete on APCs even for fixed alphabets in general, and show them to be decidable in polynomial time for fixed alphabets in this case.

==> preliminaries.tex <==

Let $\Sigma = \{a_1,\ldots, a_k\}$ be a finite set of symbols\footnote{If not otherwise stated we assume that our alphabet has
the form 
 $\Sigma = \{a_1, \ldots, a_k\}$ and $k$ denotes the number
 of symbols.},
 called an alphabet. The set $\Sigma^{\ast}$ denotes
the set of all finite sequences, i.e., of all words or strings. The finite sequence of length zero,
or the empty word, is denoted by $\varepsilon$. We set $\Sigma^+ = \Sigma^* \setminus \{\varepsilon\}$.
We call a word $u \in \Sigma^*$ a \emph{prefix} of another word $v \in \Sigma^*$,
if there exists $x \in \Sigma^*$ such that $v = ux$.
For a given word we denote by $|w|$
its length, and for $a \in \Sigma$ by $|w|_a$ the number of occurrences of the symbol $a$
in $w$. Subsets of $\Sigma^{\ast}$
are called languages. With $\mathbb N_0 = \{ 0,1,2,\ldots \}$
we denote the set of natural numbers, including zero, and $\mathbb N = \mathbb N_0 \setminus \{0\}$.
For some set $X$, by $\mathcal P(X)$ we denote the power set of $X$, i.e,
the set of all subsets of $X$. Every function $f : X \to Y$
induces a function $\hat f : \mathcal P(X) \to \mathcal P(Y)$
by setting $\hat f(Z) := \{ f(z) \mid z \in Z \}$.
Here, we will denote this extension also by $f$.
% A bijective function $f : X \to X$ is called a \emph{permutation (of $X$)}.
% If $X$ is finite, the smallest number $n \ge 0$ such that
% $f^n(x) = x$ for each $x \in X$ is called the \emph{order of the permutation}.
% Every permutation could be written uniquely as a composition of disjoint 
% cycles~\cite{cameron_1999}, then the order equals the least common multiple of all the resulting cycle
% lengths.
% By $\pi_1 : X\times Y \to X$ and $\pi_2 : X \times Y \to Y$ we denote
% the projection maps onto the first and second component, $\pi_1(x,y) = x$ and $\pi_2(x,y) = y$.
% If $a,b\in \mathbb N_0$ with $b > 0$, we denote by $a \bmod b$ the unique number $0 \le r < b$
% such that $a = bn + r$ for some $n \ge 0$.
For $n \in \mathbb N_0$ we set $[n] := \{ k \in \mathbb N_0 : 0 \le k < n \}$.
Let $M \subseteq \mathbb N_0$ be some \emph{finite} set. 
By $\max M$ we denote the maximal element in $M$
with respect to the usual order, and we set $\max \emptyset = 0$.
% Also for finite $M \subseteq \mathbb N_0 \setminus\{0\}$, i.e., $M$ is finite without zero in it,
% by $\lcm M$ we denote the
% least common multiple of the numbers in $M$, and set $\lcm \emptyset = 0$.
A \emph{finite deterministic and complete automaton} will
be denoted by $\mathcal A = (\Sigma, S, \delta, s_0, F)$
with $\delta : S \times \Sigma \to S$ the state transition function, $S$ a finite set of states, $s_0 \in S$
the start state and $F \subseteq S$ the set of final states. 
The properties of being deterministic and complete are implied by the definition of $\delta$
as a total function.
The transition function $\delta : S \times \Sigma \to S$
could be extended to a transition function on words $\delta^{\ast} : S \times \Sigma^{\ast} \to S$
by setting $\delta^{\ast}(s, \varepsilon) := s$ and $\delta^{\ast}(s, wa) := \delta(\delta^{\ast}(s, w), a)$
for $s \in S$, $a \in \Sigma$ and $w \in \Sigma^{\ast}$. In the remainder we drop
the distinction between both functions and will also denote this extension by $\delta$.
%Here we do not use
%other automata models.
% hier smei-auto einführen! todo
% A \emph{semi-automaton} $\mathcal A = (\Sigma, Q, \delta)$ 
% is like an automaton, but without a designated start state and without a set of final states.
% All (semi-)automata considered in this paper will be complete and deterministic. 
%and initially connected, the last notion meaning
%for every $s \in S$ there exists some $w \in \Sigma^{\ast}$ such that $\delta(s_0, w) = s$.
Let $\mathcal A = (\Sigma, Q, \delta, s_0, F)$ 
 be an automaton, then a trap state $t \in Q$ 
 is a state such that $\delta(t,x) = t$ for each $x \in \Sigma$.
The language accepted by $\mathcal A = (\Sigma, S, \delta, s_0, F)$ is
$
 L(\mathcal A) = \{ w \in \Sigma^{\ast} \mid \delta(s_0, w) \in F \}.
$
A language $L \subseteq \Sigma^{\ast}$ is called regular if $L = L(\mathcal A)$
for some finite automaton. 
For a language $L \subseteq \Sigma^{\ast}$ and $u, v \in \Sigma^*$
we define the Nerode right-congruence 
with respect to $L$ by $u \equiv_L v$ if and only if
$
 \forall x \in \Sigma : ux \in L \leftrightarrow vx \in L.
$
The equivalence class for some $w \in \Sigma^{\ast}$
is denoted by $[w]_{\equiv L} := \{ x \in \Sigma^{\ast} \mid x \equiv_L w \}$.
A language is regular if and only if the above right-congruence has finite index, and it could
be used to define the minimal deterministic automaton
$
 \mathcal A_L = (\Sigma, Q, \delta, [\varepsilon]_{\equiv_L}, F)
$
with $Q := \{ [w]_{\equiv_L} \mid w \in \Sigma^{\ast} \}$, $\delta([w]_{\equiv_L}, a) := [wa]_{\equiv_L}$
for $a \in \Sigma$, $w \in \Sigma^{\ast}$ and $F := \{ [w]_{\equiv_L} \mid w \in L \}$.
It is indeed the smallest automaton accepting $L$ in terms of states, and we 
will refer to this construction as the minimal automaton of $L$.
The \emph{state complexity} of a regular language
is defined as the number of Nerode right-congruence classes.
We will denote this number by $\stc(L)$.
For $u \in \Sigma^*$ and $L \subseteq \Sigma^*$, the \emph{quotient}
of $L$ by $u$ is the set $u^{-1}L = \{ v \in \Sigma^* \mid uv \in L \}$.
If $u,v \in \Sigma^*$, we have $u \equiv_L v$ if and only if $u^{-1}L = v^{-1}L$.
Hence, the quotients could be used as representatives of the Nerode equivalence classes.
Indeed, the automaton $\mathcal A = (\Sigma, Q, \delta, L, F)$
with $Q = \{ u^{-1}L \mid u \in \Sigma^* \}$, $F = \{ u^{-1}L \mid u \in \Sigma^*, \varepsilon \in u^{-1}L \}$
and $\delta(u^{-1}L, a) = (ua)^{-1}L$
is isomorphic to the minimal automaton of $L$.
Hence, $\stc(L) = |\{ u^{-1}L \mid u \in \Sigma^* \}|$ for regular $L \subseteq \Sigma^*$.
Let $\mathcal A = (\Sigma, Q, \delta, s_0, F)$ be an automaton.
A state $q \in Q$ is \emph{reachable}, if $q = \delta(s_0, u)$
for some $u \in \Sigma^*$.
Two states $q, q'$ are \emph{distinguishable},
if there exists $u \in \Sigma$ such that $|\{ \delta(q,u), \delta(q',u) \} \cap F| = 1$.
An automaton for a regular language is isomorphic to the minimal automaton
if and only if all states are reachable and distinguishable.
We will also talk about the state complexity of a %(combined)
regularity-preserving operation. 
If $f : \mathcal P(\Sigma^*)^n 
\to \mathcal P(\Sigma^*)$ is a regularity-preserving operation,
usually its state complexity is
the function $\stc(f) : \mathbb N_0^n \to \mathbb N_0$
given by 
$\stc(f)(m_1, \ldots, m_n) = \max\{ \stc(f(L_1, \ldots, L_n)) \mid L_i \mbox{ regular with } \stc(L_i) \le m_i \mbox{ for } i \in \{1,\ldots, n\} \}$. The same definition holds
for operations that are only regularity-preserving on subclasses, or if we 
are only interested in certain subclasses. Then the domain is restricted to this subclass. For example, in this work
we only look at finite languages. See~\cite{GaoMRY17}, for example, for an overview
of a wealth of subclasses of regular languages that where considered in the literature.
But here, we also allow a state complexity bound to depend on different 
parameters than merely the state complexity of the input languages, namely
later we will give a bound in terms of the lengths of the longest strings in the unary projection languages.
In that case, the state complexity function is expressed in terms of these parameters.
% Given two automata $\mathcal A = (\Sigma, S, \delta, s_0, F)$
% and $\mathcal B = (\Sigma, T, \mu, t_0, E)$, an automaton homomorphism %nochmal gucken
% $h : \mathcal A \to \mathcal B$ is a map between the state sets such that 
% for each $a \in \Sigma$ and state $s \in S$ we have
% $
%  h(\delta(s, a)) = \delta(h(s),a),
% $
% $h(s_0) = t_0$ and $h^{-1}(E) = F$. If $\mathcal B$ is a surjective homomorphic image of $\mathcal A$
% as above then $L(\mathcal B) = L(\mathcal A)$.
% The minimal deterministic automaton has the additional
% property that every accepting automaton could be homomorphically mapped onto it.
% Let $\Sigma = \{a_1, \ldots, a_k\}$ be an alphabet. 
The map $\psi : \Sigma^{\ast} \to \mathbb N_0^k$
given by $\psi(w) = (|w|_{a_1}, \ldots, |w|_{a_k})$ is called the \emph{Parikh-morphism}.
For a given word $w \in \Sigma^{\ast}$ we define $\perm(w) := \{ u \in \Sigma^{\ast} : \psi(u) = \psi(w) \}$
and for languages $L \subseteq \Sigma^{\ast}$ we set $\perm(L) := \bigcup_{w\in L} \perm(w)$.
%We also define the one-letter projection mapping $\pi_j : \Sigma^{\ast} \to \{a_j\}^{\ast}$
%by $\pi_j(w) := a_j^{|w|_{a_j}}.$ 
%A language is called \emph{commutative}
%if $\perm(L) = L$, i.e., with every word each permutation of this word is also in the language.
The language $\perm(L)$ is also called the \emph{permutational (or commutative) closure}
of $L$.


\begin{definition} The \emph{shuffle operation}, denoted by $\shuffle$, is defined by
 \begin{align*}
    u \shuffle v & := \left\{ \begin{array}{ll}
     \multirow{2}{*}{$x_1 y_1 x_2 y_2 \cdots x_n y_n  \mid$} &  u = x_1 x_2 \cdots x_n, v = y_1 y_2 \cdots y_n, \\ 
         &   x_i, y_i \in \Sigma^{\ast}, 1 \le i \le n, n \ge 1
  \end{array} \right\},
 \end{align*}
 for $u,v \in \Sigma^{\ast}$ and 
  $L_1 \shuffle L_2  := \bigcup_{x \in L_1, y \in L_2} (x \shuffle y)$ for $L_1, L_2 \subseteq \Sigma^{\ast}$.
\end{definition}

%  The shuffle operation is commutative, associative and distributive with respect
%  to union. We will use these properties without further mention. In writing formulas
%  without brackets we suppose that the shuffle operation binds stronger than the set operations,
%  and the concatenation operator has the strongest binding. 
% %  The next result
% %  appears in \cite{Pin86}.
% % 
% % \begin{restatable}[]{theorem}{commlangclosure}  
% % \label{thm::comm_lang_closure} 
% %  The class of commutative languages is closed under union, intersection, complement
% %  and the shuffle operation.
% % \end{restatable}
% % \begin{comment}
% % \begin{proof} 
% %  We have $L = \perm(L)$ iff $L = \psi^{-1}(\psi(L))$, which by surjectivity is equivalent
% %  with $L = \psi^{-1}(F)$ for some $F$, as $w \in L \Leftrightarrow \psi(w) \in F$
% %  is equivalent with $F = \psi(L)$ in this case. So if $U,V$ are commutative
% %  languages we have
% %  $U \cap V = \psi^{-1}(\psi(U)) \cap \psi^{-1}(\psi(V)) = \psi^{-1}(\psi(U) \cap \psi(V))$
% %  and similar for union. For complementation
% %  we have $\Sigma^{\ast} \setminus U = \Sigma^{\ast} \setminus \psi^{-1}(\psi(U)) = \psi^{-1}(\mathbb N^k \setminus \psi(U))$.
% %  Closure under shuffle follows from the equation $U \shuffle V = \perm(U\cdot V)$,
% %  where the inclusion $U \shuffle V \subseteq \perm(U \cdot V)$ is valid for arbitrary languages,
% %  whereas the other inclusion hold for commutative languages, but not in general.\todo{steht das nicht schon irgendwo?}
% % \qed\end{proof}
% % \end{comment}
% %
% %  The state complexity of the above operations will be a major concern of our paper.
% %  %vielleicht bemekren dass wenn parikbilder gleich, und unäre sprachen geshuffelt dann beide drin oder nicht
% %  \begin{comment}
% %  We
% %  note another property of the shuffle product for commutative languages
% %  which will be used implicitly several times.
% % 
% %  \begin{lemma}
% %   For $u, v, x, y \in \Sigma^{\ast}$, then
% %   $$
% %   | \{x,y\} \cap \perm(u) \shuffle \perm(v) | \in \{0,2\}
% %     \Leftrightarrow \psi(x) = \psi(y).
% %   $$
% %   In particular if $\psi(x) = \psi(y)$, then for commutative languages $U,V$
% %   we have either $\{x,y\} \subseteq U \shuffle V$ or $\{x,y\}\cap U \shuffle V = \emptyset$.
% %   And if $U \subseteq \{a_1\}^{\ast}$, $V \subseteq \{a_2\}$ with $a_1, a_2 \in \Sigma$ distinct,
% %   then 
% %   $
% %   | \{x,y\} \cap U \shuffle V | \in \{0,2\} 
% %   \Leftrightarrow |x|_{a_1} = |y|_{a_1} \land |x|_{a_2} = |y|_{a_2}
% %   und rest null
% %   $
% %  \end{lemma}
% % \end{comment}
% %  A regular language is called \emph{aperiodic} if it is accepted
% % by some complete automaton in which no word induces a
% % permutation of some subset of states. More formally if for all $w \in \Sigma^{\ast}$,
% % states $s \in S$ and $n \ge 1$ we have
% % $
% %  \delta(s, w^n) = s 
% % $
% % implies $\delta(s,w) = s$. Notice that by this condition all minimal cycles in the automaton
% % must be labelled by primitive words, where a word is primitive if it is not
% % a non-trivial power of another word, and conversely if a non-trivial power of a word labels
% % a minimal cycle then the above condition cannot hold. The class of aperiodic
% % languages was introduced in~\cite{McNaughton71} and admits a wealth of other
% % characterizations in terms of logic, regular expressions and other means.
% We call a language a \emph{(pure-)group language}\footnote{These were
% introduced in~\cite{McNaughton67} under the name of pure-group events.}
% if it is accepted by a complete automaton
% where every letter acts as a permutation on the state set. %tood sprechweise acts on, oder permutes the set of states
% Such automata are also called permutation automata, and the name stems
% from the fact that the transformation monoid of such an automaton forms a group. %definitionen trafo monoid, group todo. todo, def synt. monoid
% Note some ambiguity here in the sense that if $\Sigma = \{a,b\}$, then $(aa)^{\ast}$
% is not a group language over this alphabet, but it is over the unary alphabet $\{a\}$.
% Hence we mean the existence of a permutation automaton over some alphabet. By definition $\{\varepsilon\}$ is considered
% to be a group language\footnote{It is not possible
% to give such an automaton for $|\Sigma|\ge 1$,
% but allowing $\Sigma=\emptyset$ the single-state automaton
% will do, or similar as $\Sigma^{\ast} = \{\varepsilon\}$ in this case
% and $\Sigma^*$ is always a group language as witnessed by
% the complete automaton with a single accepting state.}. The next
% result is taken from~\cite{FerPSV2017} and gives 
% equations like $\perm(UV) = \perm(U) \shuffle \perm(V)$
% or $\perm(U^*) = \perm(U)^{\shuffle,*}$ for $U,V \subseteq \Sigma^*$
% that we will use frequently without special mentioning.
% %that will be used
% %without mentioning.
% %todo iterated shuffle definieren

% % , this will unify the statements
% % of some results. 
% % The next is stated (slightly different) in \cite{McNaughton71}.


% % \begin{restatable}{lemma}{aperiodicdef}
% % \label{lem::aperiodic_def}
% %  An automaton $\mathcal A = (\Sigma, S, \delta, s_0, F)$
% %  is aperiodic if and only if there exists $n \ge 0$
% %  such that for all states $s \in S$ and any
% %  word $w \in \Sigma$ we have
% %  $
% %   \delta(s, w^n) = \delta(s, w^{n+1}).
% %  $\todo{Ist das nicht bekannt? \\ SH: Ja, auf Literatur verwiesen.}
% % \end{restatable} 
% \begin{comment}
% \begin{proof} 
%  For each $w \in \Sigma^{\ast}$
%  define a function $f_w : S \to S$
%  by $f_w(s) := \delta(s, w)$.
%  Then consider the finite transformation semigroup 
%  $T := \{ f_{w} : S \to S \mid w \in \Sigma \}$
%  with function composition as operation.
%  Fix some numeration $T = \{ t_1, \ldots, t_n \}$.
%  For each $t_i \in T$
%  we consider the powers $t_i, t_i^2, t_i^3,\ldots$ 
%  and so on.
%  By finiteness we have $n_i$ and $p_i > 0$ such that
%  $t_i^{n_i + p_i} = t_i^{n_i}$. Then
%  set $n := \max\{n_1, \ldots, n_n\}$
%  and $p := \lcm\{p_1, \ldots, p_n \}$. With these numbers
%  we have $t_i^{n+p} = t_i^n$ for each $t_i$, or 
%  written in terms of the automaton we have
%  for each word $w \in \Sigma^{\ast}$ and each state $s \in S$
%  $$
%   \delta(s, w^{n+p}) = \delta(s, w^n).
%  $$
%  Fix some $s \in S$. 
%  By aperiodicity the equation $\delta(\delta(s,w^n), w^p) = \delta(s,w^n)$
%  implies $\delta(\delta(s,w^n), w) = \delta(s,w^n)$ which gives our claim.
 
 
%  Conversely assume we have some $n \ge 0$ such that
%  for each $s \in S$ and $w \in \Sigma^{\ast}$
%  we have $\delta(s, w^n) = \delta(s, w^{n+1})$. 
%  Now suppose we have some fixed state $r \in S$
%  and word $u \in \Sigma^{\ast}$ and $k > 0$
%  such that $\delta(r, u^k) = r$,
%  then we could write $\delta(r, u^{nk + k}) = r$,
%  which implies $\delta(r, u^{nk + k - i}) = r$
%  for $i = k-1, k - 2$ down to $i = 1$.
%  But by assumption $\delta(r, u^{nk}) = r$, so
%  we find $r = \delta(r, u^{nk+1}) = \delta(\delta(r, u^{nk}), u) = \delta(r,u)$.
%  As the state, word and $k > 0$ was choosen
%  arbitrary this shows that our automaton is aperiodic.
% \qed\end{proof}
% \end{comment}

% \begin{theorem}\cite{FerPSV2017}
% \label{thm:perm_semiring_hom}
%  $\perm : \mathcal P(\Sigma^*) \to \mathcal P(\Sigma^*)$
%  is a semiring morphism from the semiring
%  $(\mathcal P(\Sigma^*), \cup, \cdot, \emptyset, \{\varepsilon\})$
%  to the semiring $(\mathcal P(\Sigma^*), \cup, \shuffle, \emptyset, \{\varepsilon\})$
%  that also respects the iterated catenation resp. iterated shuffle operation.
% \end{theorem}

% Let $L \subseteq \Sigma^*$ be a commutative regular languages. 
% For each $j \in \{1, \ldots, k\}$
% let $i_j \ge 0$ and $p_j \ge 1$
% be the smallest numbers such that $[a_j^{i_j}]_{\equiv_L} = [a_j^{i_j + p_j}]$.
% The vectors $(i_1, \ldots, i_k)$
% and $(p_1, \ldots, p_k)$ are then called the \emph{index} 
% and \emph{period} vectors of $L$.
% These notions where introduced in~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20}
% and it was shown that we could bound the state complexity of $L$
% by these.

% \begin{theorem}\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20}
%  Let $L$ be a commutative regular language
%  with index vector $(i_1, \ldots, i_k)$
%  and period vector $(p_1, \ldots, p_k)$.
%  Then $\stc(L) \le \prod_{j=1}^k (i_j + p_j)$.
% \end{theorem}

% %For group languages,
% %as the minimal automaton is a permutation automaton, 
% %and by methods 
% A commutative regular language is a group languages if and only
% if its index vector is the zero vector. This follows by constructions 
% from~\cite{DBLP:conf/cai/Hoffmann19,Hoffmann20} and as 
% the minimal automaton of a group language is a permutation automaton.
% The period vector was only defined for commutative regular languages,
% but let us note that in our context it also makes sense
% to define it for group languages in general. In this case, the numbers $p_j \ge 1$
% are the smallest numbers such that $[a_j^{p_j}]_{\equiv_L} = [a_j]_{\equiv_L}$.
% As for each $w \in \Sigma^*$ we have $[w]_{\equiv_L}[a_j]_{\equiv_L} = [wa_j]_{\equiv_L}$
% and this gives a permutation on the equivalence classes,
% we find $[a_j]_{\equiv_L}^{p_j-1} = [\varepsilon]_{\equiv_L}$.
% Hence $p_j - 1$ is the order of the letter $a_j$ acting
% on the states of the minimal automaton.
%
% \subsection{Unary Languages}
% \label{sec:unary}
%
% Let $\Sigma = \{a\}$ be a unary alphabet. In this section we collect some results about unary languages.
% Suppose $L \subseteq \Sigma^{\ast}$ is regular
% with an accepting complete deterministic automaton $\mathcal A = (\Sigma, S, \delta, s_0, F)$. Then by considering
% the sequence of states $\delta(s_0, a^1), \delta(s_0, a^2), \delta(s_0, a^3), \ldots$ we find numbers $i \ge 0, p > 0$ with $i$ and $p$ minimal such that $\delta(s_0, a^i) = \delta(s_0, a^{i+p})$.
% We call these numbers the index $i$ and the period $p$ of the automaton $\mathcal A$.
% Suppose $\mathcal A$ is initially connected, i.e., $\delta(s_0, \Sigma^*) = Q$.
% Then $i+p = |S|$ and the states from $\{ s_0, \delta(s_0, a), \ldots, \delta(s_0, a^{i-1}) \}$
% constitute the \emph{tail}, and the states
% from $\{ \delta(s_0, a^i), \delta(s_0, a^{i+1}), \ldots, \delta(s_0, a^{i+p-1} \}$
% constitute the unique \emph{cycle} of the automaton.
% If $\mathcal A$ is not initially connected, when we speak of the cycle or tail
% of that automaton we nevertheless mean the above sets, despite the automaton graph
% might have more than one cycle or more than one straight path.
A language $L \subseteq \Sigma^*$ with $|\Sigma| = 1$ is called a \emph{unary language}.
For a language $L \subseteq \Sigma^*$, the languages $\{ a^{|w|_a} \mid w \in L \}$
for $a \in \Sigma$ are called the \emph{unary projection languages}.
We will need the well-known inequality of the arithmetic and
geometric mean.

\begin{theorem}{(AM-GM inequality~\cite{cauchy_2009,Aigner06})}
\label{thm:am_gm_inequality}
 Let $x_1, \ldots, x_n$ be $n$ non-negative numbers, then
 \begin{equation}\label{eqn:am_gm_inequality} 
  \sqrt[n]{x_1 \cdots x_n} \le \frac{x_1 + \ldots + x_n}{n},
 \end{equation}
 and equality holds precisely if $x_1 = x_2 = \ldots = x_n$.
\end{theorem}

For $n,m \in \mathbb N_0$,
we set $n^{\underline 0} = 1$
and $n^{\underline m} = n(n-1)\cdots (n-m+1)$ for $m > 0$. 

